UnweaveNet: Unweaving Activity Stories

Our lives can be seen as a complex weaving of activities; we switch from one activity to another, to maximise our achievements or in reaction to demands placed upon us. Observing a video of unscripted daily activities, we parse the video into its constituent activity threads through a process we call unweaving. To accomplish this, we introduce a video representation explicitly capturing activity threads called a thread bank, along with a neural controller capable of detecting goal changes and resuming of past activities, together forming UnweaveNet. We train and evaluate UnweaveNet on sequences from the unscripted egocentric dataset EPIC-KITCHENS. We propose and showcase the efficacy of pretraining UnweaveNet in a self-supervised manner.

==> Makefile <==
# You want latexmk to *always* run, because make does not have all the info.
# Also, include non-file targets in .PHONY so they are run regardless of any
# file of the given name existing.
DOC_SRC:=$(shell find . -maxdepth 1 -iregex './[^.].*\.tex')
IMG_SRC:=$(shell find figures -iname '*.svg')
IMG_TGT:=$(patsubst %.svg,%.pdf,$(IMG_SRC))
BIB_FILES:= bibliography.bib
DEPS := $(DOC_SRC) $(BIB_FILES) $(IMG_TGT)

.PHONY: all
.SECONDARY: $(PDF_SVG)

all: unweavenet.pdf

# -pdf tells latexmk to generate PDF directly (instead of DVI).
# -pdflatex="" tells latexmk to call a specific backend with specific options.
# -use-make tells latexmk to call make for generating missing files.
# -interaction=nonstopmode keeps the pdflatex backend from stopping at a
#     missing file reference and interactively asking you for an alternative.

%.pdf: %.tex #$(DEPS)
	latexmk -f -pdf -pdflatex="pdflatex -interaction=nonstopmode --shell-escape" -use-make $<

%.pdf: %.svg
# Inkscape v0.9X
#	inkscape $< --export-area-drawing --without-gui --export-type=pdf --export-file $@
# Inkscape v1.0+
	inkscape $< --export-type=pdf --export-area-page --export-dpi=600 $@

.PHONY: clean
clean:
	latexmk -C $(DOC_SRC)

